Deep Generative Models for Decision-Making and Control

Deep model-based reinforcement learning methods offer a conceptually simple approach to the decision-making and control problem: use learning for the purpose of estimating an approximate dynamics model, and offload the rest of the work to classical trajectory optimization. However, this combination has a number of empirical shortcomings, limiting the usefulness of model-based methods in practice. The dual purpose of this thesis is to study the reasons for these shortcomings and to propose solutions for the uncovered problems. Along the way, we highlight how inference techniques from the contemporary generative modeling toolbox, including beam search, classifier-guided sampling, and image inpainting, can be reinterpreted as viable planning strategies for reinforcement learning problems.

==> Makefile <==
LATEX=pdflatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

MAIN=thesis
SOURCES=$(MAIN).tex Makefile **/*.tex **/**/*.tex references.bib
FIGURES := $(shell find figures/* -type f)

all: $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
		$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
			-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
		touch .refresh
		rm $(MAIN).pdf
		$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
			-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
		$(LATEXMK) -C $(MAIN)
		rm -f $(MAIN).pdfsync
		rm -rf *~ *.tmp
		rm -f *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk

once:
		$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
		$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all

==> diffuser/figures/block_stack_joined.tex <==
\begin{figure}[t]
\begin{minipage}{0.45\textwidth}
    \centering
    \small
    \begin{tabular}{lrrr}
    \toprule
    \multicolumn{1}{c}{\textbf{Environment}} & \multicolumn{1}{c}{\textbf{~~~~~BCQ~}} &
        \multicolumn{1}{c}{\textbf{~~~~~CQL~}} &
        \multicolumn{1}{c}{\textbf{~~\method}} \\
    \midrule
    Unconditional Stacking & $0.0$ & $24.4$ & ~\highlight{\color{highlight}58.7} \scriptsize{\raisebox{1pt}{$\pm 2.5$}}
         \\ 
    Conditional Stacking & 0.0  & 0.0 & \highlight{\color{highlight}45.6} \scriptsize{\raisebox{1pt}{$\pm 3.1$}}
         \\ 
    Rearrangement & 0.0  & 0.0 & \highlight{\color{highlight}58.9} \scriptsize{\raisebox{1pt}{$\pm 3.4$}} \\ 
    \midrule
    \multicolumn{1}{c}{\textbf{Average}} & 0.0  & 8.1 & \highlight{\color{highlight}54.4~~} \hspace{.44cm} \\ 
    \bottomrule
    \end{tabular}
    % \vspace{.2cm}
    \captionof{table}{
    % \small
    % \caption{
    \textbf{(Test-time flexibility)}
    Performance of BCQ, CQL, and \method on block stacking tasks.
    A score of 100 corresponds to a perfectly executed stack; 0 is that of a random policy.
    }
    \label{table:blocks}
\end{minipage}
\begin{minipage}{0.45\textwidth}
    \centering
    % \begin{minipage}{.8\columnwidth}
    \includegraphics[width=0.3\columnwidth]{diffuser/images/blocks/blocks_0.png}
    \raisebox{1.7cm}{\hspace{0cm}$\rightarrow$}\hspace{.5cm}
    \includegraphics[width=0.3\columnwidth]{diffuser/images/blocks/blocks_1.png}
    \caption{
        \textbf{(Block stacking)}
        A block stacking sequence executed by \method. This task is best illustrated by videos viewable at
        \href{https://diffusion-planning.github.io/}
        {\texttt{diffusion-planning.github.io}}.
    }
    \label{fig:blocks}
\end{minipage}
\end{figure}

==> diffuser/text/abstract.tex <==
\begin{abstract}
Model-based reinforcement learning methods often use learning only for the purpose of estimating an approximate dynamics model, offloading the rest of the decision-making work to classical trajectory optimizers.
While conceptually simple, this combination has a number of empirical shortcomings, suggesting that learned models may not be well-suited to standard trajectory optimization.
In this paper, we consider what it would look like to fold as much of the trajectory optimization pipeline as possible into the modeling problem, such that sampling from the model and planning with it become nearly identical.
The core of our technical approach lies in a diffusion probabilistic model that plans by iteratively denoising trajectories.
We show how classifier-guided sampling and image inpainting can be reinterpreted as coherent planning strategies, explore the unusual and useful properties of diffusion-based planning methods, and demonstrate the effectiveness of our framework in control settings that emphasize long-horizon decision-making and test-time flexibility.
\end{abstract}


==> gamma/text/abstract.tex <==
\begin{abstract}
We introduce the $\gamma$-model, a predictive model of environment dynamics with an infinite probabilistic horizon.
Replacing standard single-step models with $\gamma$-models
leads to generalizations of the procedures central to model-based control, including the model rollout and model-based value estimation.
The $\gamma$-model, trained with a generative reinterpretation of temporal difference learning, is a natural continuous analogue of the successor representation and a hybrid between model-free and model-based mechanisms.
Like a value function, it contains information about the long-term future; like a standard predictive model, it is independent of task reward.
We instantiate the $\gamma$-model as both a generative adversarial network and normalizing flow, discuss how its training reflects an inescapable tradeoff between training-time and testing-time compounding errors, and empirically investigate its utility for prediction and control.
\end{abstract}



==> gamma/text/background.tex <==
\section{Preliminaries}
\label{sec:prelim}

We consider an infinite-horizon Markov decision process (MDP) defined by the tuple $(\mathcal{S}, \mathcal{A}, p, r, \gamma)$, with state space $\mathcal{S}$ and action space $\mathcal{A}$.
The transition distribution and reward function are given by $p: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \to \mathbb{R}^{+}$ and $r : \mathcal{S} \to \mathbb{R}$, respectively.
The discount is denoted by $\gamma \in (0,1)$.
A policy $\pi : \mathcal{S} \times \mathcal{A} \to \mathbb{R}^{+}$ induces a conditional occupancy $\occupancy(\bs \mid \st, \at)$ over future states:
% \newcommand{\delt}{\Delta t}

\begin{equation}
\label{eq:occupancy}
    \occupancy(\bs \mid \st, \at) = (1-\gamma) \sum_{\delt=1}^{\infty} \gammam^{\delt-1} p(\mathbf{s}_{t+\delt} = \bs \mid \st, \at, \pi).
\end{equation}

We denote parametric approximations of $p$ ($\occupancy$) as $p_\theta$ ($\model$), in which the subscripts denote model parameters.
Standard model-based reinforcement learning algorithms employ the single-step model $p_\theta$ for long-horizon decision-making by performing multi-step model-based rollouts.


==> setup/classicthesis-config.tex <==
% -*- root: thesis.tex -*-
% ****************************************************************************************************
% classicthesis-config.tex 
% formerly known as loadpackages.sty, classicthesis-ldpkg.sty, and classicthesis-preamble.sty 
% Use it at the beginning of your ClassicThesis.tex, or as a LaTeX Preamble 
% in your ClassicThesis.{tex,lyx} with \input{classicthesis-config}
% ****************************************************************************************************  
% If you like the classicthesis, then I would appreciate a postcard. 
% My address can be found in the file ClassicThesis.pdf. A collection 
% of the postcards I received so far is available online at 
% http://postcards.miede.de
% ****************************************************************************************************


% ****************************************************************************************************
% 0. Set the encoding of your files. UTF-8 is the only sensible encoding nowadays. If you can't read
% äöüßáéçèê∂åëæƒÏ€ then change the encoding setting in your editor, not the line below. If your editor
% does not support utf8 use another editor!
% ****************************************************************************************************
\PassOptionsToPackage{utf8}{inputenc}
	\usepackage{inputenc}

% ****************************************************************************************************
% 1. Configure classicthesis for your needs here, e.g., remove "drafting" below 
% in order to deactivate the time-stamp on the pages
% ****************************************************************************************************
% drafting
\PassOptionsToPackage{eulerchapternumbers,
listings,%
                    linedheaders,
					 pdfspacing,%floatperchapter,%linedheaders,%
					 subfig,beramono,eulermath,parts}{classicthesis}                                        
% ********************************************************************
% Available options for classicthesis.sty 
% (see ClassicThesis.pdf for more information):
% drafting
% parts nochapters linedheaders
% eulerchapternumbers beramono eulermath pdfspacing minionprospacing
% tocaligned dottedtoc manychapters
% listings floatperchapter subfig
% ********************************************************************


% ****************************************************************************************************
% 2. Personal data and user ad-hoc commands
% ****************************************************************************************************
\newcommand{\myTitle}{Meta Learning for Control\xspace}
\newcommand{\mySubtitle}{\xspace}
\newcommand{\myDegree}{\xspace}
\newcommand{\myName}{Yan Duan\xspace}
\newcommand{\myFaculty}{Pieter Abbeel\xspace}
\newcommand{\myDepartment}{Department of Electrical Engineering and Computer Sciences\xspace}
\newcommand{\myUni}{University of California, Berkeley\xspace}
\newcommand{\myLocation}{\xspace}
\newcommand{\myTime}{Fall, 2017\xspace}
% \newcommand{\myVersion}{version 4.2\xspace}

% ********************************************************************
% Setup, finetuning, and useful commands
% ********************************************************************
\newcounter{dummy} % necessary for correct hyperlinks (to index, bib, etc.)
\newlength{\abcd} % for ab..z string length calculation
\providecommand{\mLyX}{L\kern-.1667em\lower.25em\hbox{Y}\kern-.125emX\@}
\newcommand{\ie}{i.\,e.}
\newcommand{\Ie}{I.\,e.}
\newcommand{\eg}{e.\,g.}
\newcommand{\Eg}{E.\,g.} 
% ****************************************************************************************************


% ****************************************************************************************************
% 3. Loading some handy packages
% ****************************************************************************************************
% ******************************************************************** 
% Packages with options that might require adjustments
% ******************************************************************** 
%\PassOptionsToPackage{ngerman,american}{babel}   % change this to your language(s)
% Spanish languages need extra options in order to work with this template
%\PassOptionsToPackage{spanish,es-lcroman}{babel}
	\usepackage[american]{babel}                  

\usepackage{csquotes}
\PassOptionsToPackage{%
    backend=biber, %instead of bibtex
	%%backend=bibtex8,
    bibencoding=ascii,%
	language=american,%auto,%
    uniquename=full,
    uniquelist=false,
	%%style=numeric-comp,%
    %% style=authoryear-comp, % Author 1999, 2010
    bibstyle=authoryear,
    dashed=false, % dashed: substitute rep. author with ---
    style=authoryear,%alphabetic,
    citestyle=authoryear,%alphabetic,
    sorting=nyt, % name, year, title
    maxnames=2,
    minnames=1,
    maxcitenames=2,
    mincitenames=1,
    maxbibnames=100,%2, % default: 3, et al.
    minbibnames=100, % default: 3, et al.
    backref=true,
    giveninits=false,
    natbib=true % natbib compatibility mode (\citep and \citet still work)
}{biblatex}
    \usepackage{biblatex}
%\renewcommand*{\bibfont}{\small}
\DeclareLanguageMapping{american}{american-apa}
\usepackage{xpatch}

\xpatchbibmacro{textcite}{%
          {\usebibmacro{cite:label}%
       \setunit{%
         \global\booltrue{cbx:parens}%
         \addspace\bibopenparen}%
       \ifnumequal{\value{citecount}}{1}
         {\usebibmacro{prenote}}
         {}%
       \ifthenelse{\ifciteibid\AND\NOT\iffirstonpage}
         {\usebibmacro{cite:ibid}}
         {\usebibmacro{cite:labelyear+extrayear}}}
}{%
          {\usebibmacro{cite:label}%
       \setunit{%
         \global\booltrue{cbx:parens}%
         \addspace\bibopenparen}%
       \ifnumequal{\value{citecount}}{1}
         {\usebibmacro{prenote}}
         {}%
      \usebibmacro{cite:labelyear+extrayear}}
}{}{}

\xpatchbibmacro{textcite}{%
             {\ifthenelse{\ifciteibid\AND\NOT\iffirstonpage}
        {\usebibmacro{cite:ibid}}
        {\usebibmacro{cite:labelyear+extrayear}}}%
}{%
             {\usebibmacro{cite:labelyear+extrayear}}%
}{}{}

% \PassOptionsToPackage{fleqn}{amsmath}       % math environments and more by the AMS 
    \usepackage{amsmath}
% \setlength{\mathindent}{0cm}
% ******************************************************************** 
% General useful packages
% ******************************************************************** 
\PassOptionsToPackage{T1}{fontenc} % T2A for cyrillics
    \usepackage{fontenc}     
\usepackage{textcomp} % fix warning with missing font shapes
\usepackage{scrhack} % fix warnings when using KOMA with listings package          
\usepackage{xspace} % to get the spacing after macros right  
\usepackage{mparhack} % get marginpar right
%\usepackage[latest]{latexrelease} % will be used once available in more distributions (ISSUE #107)
\PassOptionsToPackage{printonlyused,smaller}{acronym} 
    \usepackage{acronym} % nice macros for handling all acronyms in the thesis
    %\renewcommand{\bflabel}[1]{{#1}\hfill} % fix the list of acronyms --> no longer working
    %\renewcommand*{\acsfont}[1]{\textsc{#1}} 
    \renewcommand*{\aclabelfont}[1]{\acsfont{#1}}
% ****************************************************************************************************


% ****************************************************************************************************
% 4. Setup floats: tables, (sub)figures, and captions
% ****************************************************************************************************
\usepackage{tabularx} % better tables
    \setlength{\extrarowheight}{3pt} % increase table row height
\newcommand{\tableheadline}[1]{\multicolumn{1}{c}{\spacedlowsmallcaps{#1}}}
\newcommand{\myfloatalign}{\centering} % to be used with each float for alignment
\usepackage{caption}
% Thanks to cgnieder and Claus Lahiri
% http://tex.stackexchange.com/questions/69349/spacedlowsmallcaps-in-caption-label
% [REMOVED DUE TO OTHER PROBLEMS, SEE ISSUE #82]    
%\DeclareCaptionLabelFormat{smallcaps}{\bothIfFirst{#1}{~}\MakeTextLowercase{\textsc{#2}}}
%\captionsetup{font=small,labelformat=smallcaps} % format=hang,
\captionsetup{font=small} % format=hang,
%\usepackage{subfig}  
% ****************************************************************************************************


% ****************************************************************************************************
% 5. Setup code listings
% ****************************************************************************************************
\usepackage{listings} 
%\lstset{emph={trueIndex,root},emphstyle=\color{BlueViolet}}%\underbar} % for special keywords
\lstset{language=[LaTeX]Tex,%C++,
    morekeywords={PassOptionsToPackage,selectlanguage},
    keywordstyle=\color{RoyalBlue},%\bfseries,
    basicstyle=\small\ttfamily,
    %identifierstyle=\color{NavyBlue},
    commentstyle=\color{Green}\ttfamily,
    stringstyle=\rmfamily,
    numbers=none,%left,%
    numberstyle=\scriptsize,%\tiny
    stepnumber=5,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    %frameround=ftff,
    %frame=single,
    belowcaptionskip=.75\baselineskip
    %frame=L
} 
% ****************************************************************************************************             


% ****************************************************************************************************
% 6. PDFLaTeX, hyperreferences and citation backreferences
% ****************************************************************************************************
% ********************************************************************
% Using PDFLaTeX
% ********************************************************************
\PassOptionsToPackage{pdftex,hyperfootnotes=false,pdfpagelabels}{hyperref}
    \usepackage{hyperref}  % backref linktocpage pagebackref
\pdfcompresslevel=9
\pdfadjustspacing=1 
\PassOptionsToPackage{pdftex}{graphicx}
    \usepackage{graphicx} 
 

% ********************************************************************
% Hyperreferences
% ********************************************************************
\hypersetup{%
    %draft, % = no hyperlinking at all (useful in b/w printouts)
    colorlinks=true, linktocpage=true, pdfstartpage=3, pdfstartview=FitV,%
    % uncomment the following line if you want to have black links (e.g., for printing)
    %colorlinks=false, linktocpage=false, pdfstartpage=3, pdfstartview=FitV, pdfborder={0 0 0},%
    breaklinks=true, pdfpagemode=UseNone, pageanchor=true, pdfpagemode=UseOutlines,%
    plainpages=false, bookmarksnumbered, bookmarksopen=true, bookmarksopenlevel=1,%
    hypertexnames=true, pdfhighlight=/O,%nesting=true,%frenchlinks,%
    urlcolor=webbrown, linkcolor=RoyalBlue, citecolor=berkeleyblue, %pagecolor=RoyalBlue,%
    %urlcolor=Black, linkcolor=Black, citecolor=Black, %pagecolor=Black,%
    pdftitle={\myTitle},%
    pdfauthor={\textcopyright\ \myName, \myUni, \myFaculty},%
    pdfsubject={},%
    pdfkeywords={},%
    pdfcreator={pdfLaTeX},%
    pdfproducer={LaTeX with hyperref and classicthesis}%
}   

% ********************************************************************
% Setup autoreferences
% ********************************************************************
% There are some issues regarding autorefnames
% http://www.ureader.de/msg/136221647.aspx
% http://www.tex.ac.uk/cgi-bin/texfaq2html?label=latexwords
% you have to redefine the makros for the 
% language you use, e.g., american, ngerman
% (as chosen when loading babel/AtBeginDocument)
% ********************************************************************
\makeatletter
%\usepackage[english]{babel}

\@ifpackageloaded{babel}%
    {%
       \addto\extrasamerican{%
			\renewcommand*{\figureautorefname}{Figure}%
			\renewcommand*{\tableautorefname}{Table}%
			\renewcommand*{\partautorefname}{Part}%
			\renewcommand*{\chapterautorefname}{Chapter}%
			\renewcommand*{\sectionautorefname}{Section}%
			\renewcommand*{\subsectionautorefname}{Section}%
			\renewcommand*{\subsubsectionautorefname}{Section}%     
                }%
       \addto\extrasngerman{% 
			\renewcommand*{\paragraphautorefname}{Absatz}%
			\renewcommand*{\subparagraphautorefname}{Unterabsatz}%
			\renewcommand*{\footnoteautorefname}{Fu\"snote}%
			\renewcommand*{\FancyVerbLineautorefname}{Zeile}%
			\renewcommand*{\theoremautorefname}{Theorem}%
			\renewcommand*{\appendixautorefname}{Anhang}%
			\renewcommand*{\equationautorefname}{Gleichung}%        
			\renewcommand*{\itemautorefname}{Punkt}%
                }%  
            % Fix to getting autorefs for subfigures right (thanks to Belinda Vogt for changing the definition)
            \providecommand{\subfigureautorefname}{\figureautorefname}%             
    }{\relax}
\makeatother


% ****************************************************************************************************
% 7. Last calls before the bar closes
% ****************************************************************************************************
% ********************************************************************
% Development Stuff
% ********************************************************************
\listfiles
%\PassOptionsToPackage{l2tabu,orthodox,abort}{nag}
%   \usepackage{nag}
%\PassOptionsToPackage{warning, all}{onlyamsmath}
%   \usepackage{onlyamsmath}

% ********************************************************************
% Last, but not least...
% ********************************************************************
\usepackage{classicthesis} 
% ****************************************************************************************************


% ****************************************************************************************************
% 8. Further adjustments (experimental)
% ****************************************************************************************************
% ********************************************************************
% Changing the text area
% ********************************************************************
%\linespread{1.05} % a bit more for Palatino
%\areaset[current]{312pt}{761pt} % 686 (factor 2.2) + 33 head + 42 head \the\footskip
%\setlength{\marginparwidth}{7em}%
%\setlength{\marginparsep}{2em}%

% ********************************************************************
% Using different fonts
% ********************************************************************
%\usepackage[oldstylenums]{kpfonts} % oldstyle notextcomp
%\usepackage[osf]{libertine}
%\usepackage[light,condensed,math]{iwona}
%\renewcommand{\sfdefault}{iwona}
%\usepackage{lmodern} % <-- no osf support :-(
%\usepackage{cfr-lm} % 
%\usepackage[urw-garamond]{mathdesign} <-- no osf support :-(
%\usepackage[default,osfigures]{opensans} % scale=0.95 
%\usepackage[sfdefault]{FiraSans}
% ****************************************************************************************************


==> transformer/figures/imitation.tex <==
\begin{wrapfigure}[18]{r}{0.35\linewidth}
    \vspace{-0.25cm}
    \centering 
    \includegraphics[width=0.98\linewidth]{images/imitation.pdf}
    \caption{
    \textbf{(Imitation learning)}
    We find that TTO, despite being built on the tools of natural language processing instead of behvior cloning, is a capable imitative method.
    Performance of the behavior cloning (BC) baseline is taken from \citep{kumar2020conservative}.
    }
    \label{fig:imitation}
\end{wrapfigure}


==> transformer/text/abstract.tex <==
\begin{abstract}
Reinforcement learning (RL) is typically concerned with estimating stationary policies or single-step models, leveraging the Markov property to factorize problems in time.
However, we can also view RL as a generic sequence modeling problem, with the goal being to produce a sequence of actions that leads to a sequence of high rewards.
Viewed in this way, it is tempting to consider whether high-capacity sequence prediction models that work well in other domains, such as natural-language processing, can also provide effective solutions to the RL problem.
To this end, we explore how RL can be tackled with the tools of sequence modeling, using a Transformer architecture to model distributions over trajectories and repurposing beam search as a planning algorithm.
Framing RL as sequence modeling problem simplifies a range of design decisions, allowing us to dispense with many of the components common in offline RL algorithms.
We demonstrate the flexibility of this approach across long-horizon dynamics prediction, imitation learning, goal-conditioned RL, and offline RL.
Further, we show that this approach can be combined with existing model-free algorithms to yield a state-of-the-art planner in sparse-reward, long-horizon tasks.
\blfootnote{
Code is available at
    \href{https://trajectory-transformer.github.io/}
    {\texttt{trajectory-transformer.github.io}}
\vspace{-.4cm}}
\end{abstract}

